Multi-Label Class Balancing Algorithm for Action Unit Detection

Isolated facial movements, so-called Action Units, can describe combined emotions or physical states such as pain. As datasets are limited and mostly imbalanced, we present an approach incorporating a multi-label class balancing algorithm. This submission is subject to the Action Unit detection task of the Affective Behavior Analysis in-the-wild (ABAW) challenge at the IEEE Conference on Face and Gesture Recognition 2020.

==> discussion.tex <==
\section{Discussion}
%discuss shortly, why some aus are not so well detected
